Towards Practicable Algorithms for Rewriting Graph Queries beyond DL-Lite

Despite the many advantages that ontology-based data access (OBDA) has brought to a range of application domains, state-of-the-art OBDA systems still do not support popular graph database management systems such as Neo4j. Algorithms for query rewriting focus on languages like conjunctive queries and their unions, which are fragments of first-order logic and were developed for relational data. Such query languages are poorly suited for querying graph data. Moreover, they also limit the expressiveness of the ontology languages that admit rewritings, restricting them to those where the data complexity of reasoning is not higher than it is in first-order logic. In this paper, we propose a technique for rewriting a family of navigational queries for a suitably restricted fragment of ELHI that extends DL-Lite and that is NL-complete in data complexity. We implemented a proof-of-concept prototype that rewrites into Cypher queries, and tested it on a real-world cognitive neuroscience use case with promising results.

==> 6-complexity <==
\section{Complexity bounds for $\ontoLang$}\label{sec:complexity}

From the previous sections and the data complexity for C2RPQs \cite{Barcelo2013} we get the following upper bound results.

\begin{theorem}
    NCQ answering for $\ontoLang$ is in \NL in data complexity and \textsc{ExpTime} in combined complexity.
\end{theorem}
\begin{itemize}
    \item upper bound for data complexity follows from the rewriting into UC2RPQs
    \item the combined complexity follows either from the literature since C2RPQ answering over $\mathcal{ELHI}_\bot$ is in \textsc{ExpTime} or from the complexity of \Cref{algo:rewriteC2RPQ}
\end{itemize} 

\begin{theorem}
    NCQ answering is NL-hard in data complexity for $\ontoLang$.
\end{theorem}

\begin{proof}
    reduction from the NL-complete directed reachability problem \cite{Consens1990} (equivalent to the proof in \cite{Bienvenu2013}): it holds already for a single NCQ of the form $r^*(x,y)$
\end{proof}

\begin{theorem}
    NCQ answering is Exp-hard in combined complexity for $\ontoLang$.
\end{theorem}

\begin{proof}
    reduction from Exp-hard word problem for \emph{Alternating Turing Machines} (ATMs) with polynomial space \cite{Chandra1985} (similar to the proof for N2RPQ answering in \cite{Bienvenu2014}) 
    proof idea: 
    \begin{itemize}
        \item in the proof for N2RPQs in \cite{Bienvenu2014} there is no Kleene Star over nested queries, does this mean we can come up with equivalent C2RPQs for these N2RPQs?
    \end{itemize}
\end{proof}


